Traces of intertwining operators and Macdonald's polynomials

Let $\Phi:V\to V\otimes U$ be an intertwining operator between representations of a simple Lie algebra (quantum group, affine Lie algebra). We define its generalized character to be the following function on the Cartan subalgebra with values in $U$: $\chi_\Phi(h)=\Tr_V (\Phi e^h)$. These generalized characters are a rich source of special functions, possessing many interesting properties; for example, they are common eigenfunctions of a family of commuting differential (difference) operators. We show that the special functions that can be obtained this way include Macdonald's polynomials of type $A$, and this technique allows to prove inner product and symmetry identities for these polynomials (though proved earlier by other methods). Generalized characters for affine Lie algebras are closely related with so-called correlation functions on the torus in the Wess-Zumino-Witten (WZW) model of conformal field theory. We derive differential equations satisfied by these correlation functions (elliptic Knizhnik-Zamolodchikov, or Knizhnik-Zamolodchikov-Bernard equations) and study their monodromies.

==> topmatter.tex <==
%&amstex
\input head2
\hcorrection{0.2truein}
\topmatter
\NoPageNumbers 
\endtopmatter
\document
\baselineskip 20pt



\vbox{\vskip 0.5in}
\specialhead 

\centerline{Abstract} 
\centerline{\bf Traces of intertwining operators and Macdonald's
polynomials}
\centerline{Alexander A. Kirillov, Jr.}
\centerline{ May 1995}


\endspecialhead

\vbox{\vskip 0.5in}

Let $\Phi:V\to V\o U$ be an intertwining operator between
representations of a simple Lie algebra (quantum group, affine Lie
algebra). We define its generalized character to be the following
function on the Cartan subalgebra with values in $U$:
 $\chi_\Phi(h)=\Tr_V (\Phi e^h)$. This is a generalization of usual
characters. These generalized characters are a rich
source of special functions, possessing many interesting properties;
for example, they are common eigenfunctions of a family of commuting
differential (difference) operators. We show that the special
functions that can be obtained this way include Macdonald's
polynomials of type $A$, and this technique allows to prove inner
product and symmetry identities for these polynomials (though proved
earlier by other methods). 

Generalized characters for affine Lie algebras are closely related
with so-called correlation functions on the torus in the
Wess-Zumino-Witten (WZW) model of conformal field theory. We derive
differential equations satisfied by these correlation functions
(elliptic Knizhnik-Zamolodchikov, or
Knizhnik-Zamolodchikov-Bernard  equations) and study their
monodromies. 


\vfill\newpage

\vbox{\vskip 2in}
\vfill\newpage


\vbox{\vskip 1cm}
\centerline{\bf Traces of intertwining operators and Macdonald's
polynomials}

\vskip 3cm
\centerline{A Dissertation}
\centerline{Presented to the Faculty of the Graduate School} 
\centerline{of}
\centerline{Yale University}
\centerline{in Candidacy for the Degree of}
\centerline{Doctor of Philosophy}

\vskip 4cm
\centerline{by}
\centerline{Alexander A. Kirillov, Jr.}

\vskip 1cm
\centerline{Dissertation Director: Professor Igor B. Frenkel}

\vskip 1cm
\centerline{ May 1995}

\vfill\newpage

\vbox{\vskip 7cm}

\centerline{\copyright 1995 by Alexander A. Kirillov}
\centerline{All rights reserved}

\vfill\newpage


\vbox{\vskip 1in}
\specialhead
\centerline{CONTENTS} 
\endspecialhead

\vbox{\vskip 0.5in}

\toc
\widestnumber\head{5.5}
\title Acknowledgements\page{1}\endtitle
\title Introduction \page{2}\endtitle
\title\chapter{1} Basic definitions\endtitle
\head 1.1  Simple Lie algebras and their representations\page{5} \endhead
\head 1.2 Quantum groups \page{9}\endhead
\title\chapter{2} Generalized characters\endtitle	
\head 2.1 Weighted traces of intertwiners and orthogonality theorem
	 \page{13}\endhead
\head 2.2 Center of $U\g$ and commuting differential operators\page{15}\endhead
\head 2.3 Center of $\Ug$ and difference operators \page{18}\endhead
\head 2.4 Generalized characters as spherical functions\page{20}\endhead
\title \chapter{3}Jacobi polynomials \endtitle	
\head 3.1 Jacobi polynomials and corresponding differential operators
	\page{24}\endhead
\head 3.2 Jack polynomials as generalized characters\page{27}\endhead
\title\chapter{4} Macdonald's polynomials as generalized cha\-ra\-cters
	 \endtitle	

\head 4.1 Definition of Macdonald's polynomials\page{30}\endhead
\head 4.2 Macdonald's polynomials of type $A$ as generalized characters
	\page{32}\endhead
\head 4.3 The center of $U_q\sln$ and Macdonald's operators\page{35}\endhead
\title\chapter{5} Inner product and symmetry identities for Macdonald's
	polynomials  \endtitle	
\head 5.1 Inner product identities \page{38}\endhead
\head 5.2 Algebra of intertwiners\page{41}\endhead
\head 5.3 Symmetry identities\page{48}\endhead
\title\chapter{6} Generalized characters for affine Lie algebras
	 \endtitle	
\head 6.1 Affine Lie algebras\page{51}\endhead
\head 6.2 Group algebra of the weight lattice\page{53}\endhead
\head 6.3 Generalized characters for affine Lie algebras\page{56}\endhead
\title\chapter{7} Affine Jacobi polynomials \endtitle	
\head 7.1 Definition of affine Jacobi polynomials\page{60}\endhead
\head 7.2 Affine Jack polynomials as generalized characters\page{64}\endhead
\title\chapter{8} Modular properties of affine Jacobi polynomials
	\endtitle	
\head 8.1 Functional interpretation of $\C[\Phat]$ \page{67}\endhead
\head 8.2 Normalized characters and modular invariance\page{70}\endhead
\title\chapter{9} Correlation functions on the torus and elliptic KZ
	equations \endtitle	
\head 9.1 Intertwiners and currents\page{75}\endhead
\head 9.2 Correlation functions on the torus and differential equations
	 \page{79}\endhead
\head 9.3 Monodromies of elliptic KZ equations\page{86}\endhead
\title\chapter{10} Perspectives and open questions \page{93}\endtitle	
\title Appendix: List of formulas related to elliptic
	functions  \page{95}\endtitle	
\title References\page{97}\endtitle
\endtoc


\enddocument\end








